MapFormer: Boosting Change Detection by Using Pre-change Information

Change detection in remote sensing imagery is essential for a variety of applications such as urban planning, disaster management, and climate research. However, existing methods for identifying semantically changed areas overlook the availability of semantic information in the form of existing maps describing features of the earth's surface. In this paper, we leverage this information for change detection in bi-temporal images. We show that the simple integration of the additional information via concatenation of latent representations suffices to significantly outperform state-of-the-art change detection methods. Motivated by this observation, we propose the new task of *Conditional Change Detection*, where pre-change semantic information is used as input next to bi-temporal images. To fully exploit the extra information, we propose *MapFormer*, a novel architecture based on a multi-modal feature fusion module that allows for feature processing conditioned on the available semantic information. We further employ a supervised, cross-modal contrastive loss to guide the learning of visual representations. Our approach outperforms existing change detection methods by an absolute 11.7\% and 18.4\% in terms of binary change IoU on DynamicEarthNet and HRSCD, respectively. Furthermore, we demonstrate the robustness of our approach to the quality of the pre-change semantic information and the absence pre-change imagery. The code is available at https://github.com/mxbh/mapformer.

==> Figures/attention.tex <==
\begin{figure}[t]
    \centering
    \begin{subfigure}{\columnwidth}
        \centering
        \begin{subfigure}{0.33\columnwidth}
            \subcaption*{$I_1$}
            \includegraphics[width=\columnwidth]{Figures/Examples/Attention/img_pre.png}
        \end{subfigure} \hspace{-1em}
        \begin{subfigure}{0.33\columnwidth}
            \subcaption*{$m_1$}
            \includegraphics[width=\columnwidth]{Figures/Examples/Attention/gt_sem_pre.png}
        \end{subfigure} \hspace{-1em}
        \begin{subfigure}{0.33\columnwidth}
             %\subcaption{$b$ vs $\hat{b}$ (white=true positive, black=true negative, red=false positive, blue=false negative)}
            \subcaption*{$b$ vs $\hat{b}$ (\textcolor{lightgray}{TP}, \textcolor{black}{TN},\textcolor{red}{FP},\textcolor{blue}{FN})}
            \includegraphics[width=\columnwidth]{Figures/Examples/Attention/bc.png}
        \end{subfigure}
    \end{subfigure}
    \vspace{-1.7em}
    
    \begin{subfigure}{\columnwidth}
        \centering
        \begin{subfigure}{0.33\columnwidth}
            \includegraphics[width=\columnwidth]{Figures/Examples/Attention/img_post.png}
            \subcaption*{$I_2$}
        \end{subfigure} \hspace{-1em}
        \begin{subfigure}{0.33\columnwidth}
            \includegraphics[width=\columnwidth]{Figures/Examples/Attention/gt_sem_post.png}
            \subcaption*{$m_2$}
        \end{subfigure} \hspace{-1em}
        \begin{subfigure}{0.33\columnwidth}
            \includegraphics[width=\columnwidth]{Figures/Examples/Attention/pred_sem.png}
            \subcaption*{$m^{(1)} \cdot (1 - \hat{b}) + \hat{m}^{(2)} \cdot \hat{b}$}
        \end{subfigure}
    \end{subfigure}

    \begin{subfigure}{\columnwidth}
     \centering
        \includegraphics[width=0.25\columnwidth]{Figures/Examples/Attention/attn_128_36.png} \hspace{-1em}
        \includegraphics[width=0.25\columnwidth]{Figures/Examples/Attention/attn_128_10.png} \hspace{-1em}
        \includegraphics[width=0.25\columnwidth]{Figures/Examples/Attention/attn_128_64.png} \hspace{-1em}
        \includegraphics[width=0.25\columnwidth]{Figures/Examples/Attention/attn_128_2.png}
        \subcaption*{Attention visualizations}
    \end{subfigure}
    
    \caption{Qualitative Results on DynamicEarthNet.}
    \label{fig:attention}
\end{figure}


==> Tables/ablations.tex <==
\begin{table}
\begin{tabular}{c|cc|cc}
\hline
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{DynEarthNet}} & \multicolumn{2}{c}{\textbf{HRSCD}} \\
 & \textbf{IoU} & \textbf{$\Delta$} & \textbf{IoU} & \textbf{$\Delta$} \\ \hline
Ours (full)         & 23.5 & -- & 47.2 & -- \\
\hline
\textit{\underline{Architectural Ablations:}} &  &  &  & \\ 
K=5                 & 21.1 & -2.4 & 48.0 & +0.8 \\ 
K=15                & 22.2 & -1.3 & 47.6 & +0.4 \\ 
w/o contr. loss     & 20.9 & -2.6 & 46.8 & -0.4 \\ 
w/o stop gradient   & 22.5 & -1.0 & 45.4 & -1.8 \\ 
\hline
\textit{\underline{Data Ablations:}} &  &  &  & \\ 
low resolution sem. info    & 17.9 & -5.6 & 43.2 & -4.0 \\ 
high-level sem. info        & 17.6 & -5.9 & 47.5 & +0.3 \\ 
\hline
\end{tabular}
\caption{Ablations for binary change detection.}
\label{tab:ablations}
\end{table}

==> Tables/bc.tex <==
\begin{table}
\centering
\begin{tabular}{@{\hspace{0em}}c@{\hspace{0.1em}}|c@{\hspace{1em}}c|c@{\hspace{1em}}c}
\hline
\multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{c|}{\textbf{DynENet}} & \multicolumn{2}{c}{\textbf{HRSCD}} \\
  & \textbf{F1} & \textbf{IoU} & \textbf{F1} & \textbf{IoU} \\ \hline
\textbf{\textit{\underline{Bi-temporal BCD:}}} &  &  &  & \\
SegFormer~\cite{segformer}       & 20.3 & 11.3 & 17.8 & \enskip 9.7 \\
Concatenation                    & 20.7 & 11.6 & 41.2 & 25.9 \\
FHD~\cite{fhd}                   & 17.2 & \enskip 9.4 & 45.2 & 29.2 \\ 
ChangerEx~\cite{changer}         & 21.1 & 11.8 & 37.0 & 22.7 \\
ChangeFormer~\cite{changeformer} & 20.7 & 11.5 & \underline{45.7} & \underline{29.6} \\
Ours$_{K=10}$ (w/o sem. input)     & \underline{28.6} & \underline{16.7} & 43.9 & 28.2 \\
%Ours (K=10, w/o sem info, w/o contrastive)        & 27.5 & 23.3 & 25.2 & 14.4 & 43.3 & 44.1 & 43.7 & 27.9 \\
%TODO &  &  &  &  &  &  &  &  \\ %\hline
\hline
\textbf{\textit{\underline{Conditional BCD:}}} &  &  &  & \\ 
SegFormer~\cite{segformer}       &  21.2  &  11.9   & \enskip 5.6 & \enskip 2.8 \\
Concatenation                    &  33.5  &  20.1   & 62.1 & 45.1 \\   
DynamicMLP~\cite{dynamicmlp}     &  34.5  &  20.8   & 62.7 & 45.7 \\
Ours$_{K=5}$ & 34.8 & 21.1 & \textbf{64.9} & \textbf{48.0} \\
Ours$_{K=10}$                    & \textbf{38.0}   & \textbf{23.5}    & 64.5 & 47.7 \\
Ours$_{K=15}$& 36.4 & 22.2 & 64.5 & 47.6 \\[5pt]
% -------------------------------------------------------------------------------
%\cline{1-1}
\textit{\underline{Ablations:}} &  &  &  & \\ 
Ours$_{K=10}$ (w/o constrastive)  &  34.5  &  20.9   & 63.8 &  46.8 \\
Ours$_{K=10}$ (w/o stop-gradient) &  36.7  & 22.5    & 62.5 &  45.4 \\
Ours$_{K=10}$ (w/ map proj.)       &  35.8  & 21.8    & 60.7 &  45.9 \\
%\textit{\underline{Data Ablations:}} &  &  &  &  &  &  &  &  \\ 
Ours$_{K=10}$ (high-level info)& 29.8 & 17.6 & 64.4 & 47.5 \\
Ours$_{K=10}$ (low-res. info)  & 30.4 & 17.9 & 60.3 & 43.2 \\
% -------------------------------------------------------------------------------
%Ours$_{K=5}$ (w/o constrastive)  & 32.6 & 35.1 &  33.8  &  20.3   & 75.8    & 53.8    & 62.9 &  45.9 \\
%Ours$_{K=15}$ (w/o constrastive) & 32.8 & 38.8 &  35.5  &  21.6   & 74.5    & 56.3    & 64.1 &  47.2 \\
%Ours$_{K=10}$ (w/o constrastive, high-level info) & 34.0 & 23.0 & 27.4 & 15.9 & 75.1 & 53.0 & 62.1 & 45.1 \\ 
%Ours$_{K=10}$ (w/o constrastive, low-res. info)   & 30.8 & 25.5 & 27.9 & 16.2 & 70.4 & 49.2 & 57.9 & 40.8 \\
% -------------------------------------------------------------------------------
\hline
% \textbf{\textit{\underline{Cross-modal BCD:}}} &  &  &  & \\ 
% Concatenation  & 31.8 & 18.9 & 61.5 & 44.4 \\ 
% Ours $_{K=10}$ & 32.0 & 19.0 & 62.1 & 45.0 \\
% %Ours$_{K=10}$ (w/o constrastive)   & 25.5 & 45.7 & 32.7 & 19.5 & 74.8 & 53.6 & 62.4 & 45.4 \\ 
% \hline
\end{tabular}
\caption{(Conditional) Binary Change Detection as well as ablations. Our method performs best and is still highly competitive without ground-truth semantic input.}
\label{tab:bc}
\end{table}

==> Tables/bc_pre_rec_.tex <==
\begin{table*}
\centering
\begin{tabular}{c|cccc|cccc}
\hline
\multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c|}{\textbf{DynamicEarthNet}} & \multicolumn{4}{c}{\textbf{HRSCD}} \\
 & \textbf{Prec} & \textbf{Rec} & \textbf{F1} & \textbf{IoU} & \textbf{Prec} & \textbf{Rec} & \textbf{F1} & \textbf{IoU} \\ \hline
\textbf{\textit{\underline{Bi-temporal BCD:}}} &  &  &  &  &  &  &  &  \\
Concatenation                    & 48.3 & 13.2 & 20.7 & 11.6 & 63.9 & 30.4 & 41.2 & 25.9 \\
SegFormer~\cite{segformer}       & 13.6 & 40.4 & 20.3 & 11.3 & 10.8 & 50.4 & 17.8 & \enskip 9.7 \\
FHD~\cite{fhd}                   & 11.1 & 38.1 & 17.2 & \enskip 9.4 & 44.7 & 45.7 & 45.2 & 29.2 \\ 
ChangerEx~\cite{changer}         & 36.1 & 14.9 & 21.1 & 11.8 & 37.4 & 36.7 & 37.0 & 22.7 \\
ChangeFormer~\cite{changeformer} & 40.5 & 13.9 & 20.7 & 11.5 & 43.3 & 48.4 & 45.7 & 29.6 \\
Ours$_{K=10}$ (w/o sem info)        & 31.9 & 25.9 & 28.6 & 16.7 & 45.6 & 42.4 & 43.9 & 28.2 \\
%Ours (K=10, w/o sem info, w/o contrastive)        & 27.5 & 23.3 & 25.2 & 14.4 & 43.3 & 44.1 & 43.7 & 27.9 \\
%TODO &  &  &  &  &  &  &  &  \\ %\hline
\hline
\textbf{\textit{\underline{Conditional BCD:}}} &  &  &  &  &  &  &  &  \\ 
Concatenation                    & 32.6 & 34.4 &  33.5  &  20.1   & 75.5 & 52.8    & 62.1 &  45.1 \\
DynamicMLP~\cite{dynamicmlp}    & 32.2 & 37.1 &  34.5  &  20.8   & 73.6 & 54.6 & 62.7 & 45.7 \\
Ours$_{K=5}$ & 33.1 & 36.7 & 34.8 & 21.1 & 75.1 & 57.1 & 64.9 & 48.0 \\
Ours$_{K=10}$& 37.1 & 39.0 & 38.0 & 23.5 & 76.0 & 55.5 & 64.2 & 47.2 \\
Ours$_{K=15}$& 31.5 & 43.0 & 36.4 & 22.2 & 73.1 & 57.7 & 64.5 & 47.6 \\
% -------------------------------------------------------------------------------
\cline{1-1}
\textit{\underline{Ablations:}} &  &  &  &  &  &  &  &  \\ 
Ours$_{K=10}$ (w/o constrastive)  & 34.5 & 34.5 &  34.5  &  20.9   & 73.2    & 56.5    & 63.8 &  46.8 \\
Ours$_{K=10}$ (w/o stop-gradient) & 34.8 & 38.9 &  36.7  & 22.5    & 73.8    & 54.2    & 62.5 &  45.4 \\
Ours$_{K=10}$ (w/ map proj)       & 32.4 & 40.1 &  35.8  & 21.8    & 75.1    & 51.0    & 60.7 &  45.9 \\
%\textit{\underline{Data Ablations:}} &  &  &  &  &  &  &  &  \\ 
Ours$_{K=10}$ (high-level info)& 45.8 & 22.1 & 29.8 & 17.6 & 67.9 & 61.3 & 64.4 & 47.5 \\
Ours$_{K=10}$ (low-res. info)  & 33.0 & 28.1 & 30.4 & 17.9 & 66.8 & 55.0 & 60.3 & 43.2 \\
% -------------------------------------------------------------------------------
%Ours$_{K=5}$ (w/o constrastive)  & 32.6 & 35.1 &  33.8  &  20.3   & 75.8    & 53.8    & 62.9 &  45.9 \\
%Ours$_{K=15}$ (w/o constrastive) & 32.8 & 38.8 &  35.5  &  21.6   & 74.5    & 56.3    & 64.1 &  47.2 \\
%Ours$_{K=10}$ (w/o constrastive, high-level info) & 34.0 & 23.0 & 27.4 & 15.9 & 75.1 & 53.0 & 62.1 & 45.1 \\ 
%Ours$_{K=10}$ (w/o constrastive, low-res. info)   & 30.8 & 25.5 & 27.9 & 16.2 & 70.4 & 49.2 & 57.9 & 40.8 \\
% -------------------------------------------------------------------------------
\hline
\textbf{\textit{\underline{Cross-modal CD:}}} &  &  &  &  &  &  &  &  \\ Concatenation & 25.6 & 42.1 & 31.8 & 18.9 & 75.0 & 52.1 & 61.5 & 44.4 \\ 
Ours $_{K=10}$ & 24.0 & 47.8 & 32.0 & 19.0 & 74.7 & 53.1 & 62.1 & 45.0 \\
%Ours$_{K=10}$ (w/o constrastive)   & 25.5 & 45.7 & 32.7 & 19.5 & 74.8 & 53.6 & 62.4 & 45.4 \\ 
\hline
\end{tabular}
\caption{(Conditional) Binary Change Detection.}
\label{tab:bc}
\end{table*}

==> Tables/cross_modal_bc+scd.tex <==
\begin{table*}
    \begin{minipage}{0.34\linewidth}
        %\begin{table}
            %\centering
            \begin{tabular}{@{\hspace{0.1em}}c@{\hspace{0.2em}}|@{\hspace{0.4em}}c@{\hspace{0.8em}}c@{\hspace{0.4em}}|@{\hspace{0.4em}}c@{\hspace{0.8em}}c@{\hspace{0.2em}}}
            \hline
            \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{@{\hspace{0.4em}}c@{\hspace{0.6em}}|@{\hspace{0.4em}}}{\textbf{DynENet}} & \multicolumn{2}{@{\hspace{0.4em}}c@{\hspace{0.4em}}}{\textbf{HRSCD}} \\
              & \textbf{F1} & \textbf{IoU} & \textbf{F1} & \textbf{IoU} \\ \hline
            %\textbf{\textit{\underline{Cross-modal BCD:}}} &  &  &  & \\ 
            SegFormer\,\cite{segformer}       &  21.2  &  11.9   & \enskip 5.6 & \enskip 2.8 \\
            Concatenation  & 31.8 & 18.9 & 61.5 & 44.4 \\ 
            Ours $_{K=10}$ & \textbf{32.0} & \textbf{19.0} & \textbf{62.1} & \textbf{45.0} \\
            %Ours$_{K=10}$ (w/o constrastive)   & 25.5 & 45.7 & 32.7 & 19.5 & 74.8 & 53.6 & 62.4 & 45.4 \\ 
            \hline
            \end{tabular}
            \caption{Cross-modal Binary Change Detection. Our method and the concatenation baseline clearly outperform SegFormer.}
            \label{tab:cross-modal-bc}
        %\end{table}
    \end{minipage} 
    \hfill
    \begin{minipage}{.63\linewidth}
        %\begin{table*}
        \hfill
        \begin{tabular}{@{\hspace{0.1em}}c@{\hspace{0.2em}}|@{\hspace{0.4em}}c@{\hspace{0.8em}}c@{\hspace{0.8em}}c@{\hspace{0.4em}}c@{\hspace{0.2em}}|@{\hspace{0.4em}}c@{\hspace{0.8em}}c@{\hspace{0.8em}}c@{\hspace{0.4em}}c@{\hspace{0.1em}}}
            \hline
            \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c|@{\hspace{0.4em}}}{\textbf{DynamicEarthNet}} & \multicolumn{4}{c}{\textbf{HRSCD}} \\
             & \textbf{BC} & \textbf{SC} & \textbf{SCS} & \textbf{mIoU} & \textbf{BC} & \textbf{SC} & \textbf{SCS} & \textbf{mIoU} \\ \hline
            SegFormer~\cite{segformer}    & 11.3 & \textbf{31.5} & 21.4 & 39.7 & \enskip 9.7 & 20.3 & 15.0 & 52.7 \\
            %Concatenation (Baseline) \\ \hline
            %----------------------------------------
            Ours (sem.~seg.~on~$f^{(2)}$) & 23.0 & 29.0 & \textbf{26.0} & 39.9 & 48.0 & 21.5 & \textbf{34.7} & 52.9 \\
            Ours (sem.~seg.~on~$f$)       & \textbf{23.1} & 13.1 & 18.1 & 61.5 & \textbf{48.2} & 12.5 & 30.4 & \textbf{72.3} \\
            Ours (Cross-modal~SCD)         & 20.4 & 30.7 & 25.5 & \textbf{40.3} & 45.6 & \textbf{21.7} & 33.5 & 49.9 \\
            %----------------------------------------
            %Joint Head (w/o contrastive)             & 18.9 & 15.3 & 17.1 & 60.9 & 45.0 & 11.0 & 28.0 & 70.4 \\
            %Separate Heads (w/o contrastive)         & 22.5 & 28.4 & 25.4 & 39.6 & 48.1 & 21.0 & 34.5 & 52.3 \\
            %Map Updating (uni-temp., w/o contrastive) & 20.7 & 28.8 & 24.7 & 40.0 & 46.4 & 20.9 & 33.6 & 52.3 \\
            \hline
        \end{tabular}
        \caption{(Conditional) Semantic Change Detection. Predicting $\hat{m}^{(2)}$ based on $f^{(2)}$ yields the best results w.r.t.~the main objective SCS.}
        \label{tab:scd}
        %\end{table*}
    \end{minipage} 
\end{table*}

==> Tables/rebuttal/semseg_baselines+cond_cd_baselines.tex <==
\begin{table*}
    \hfill
    \begin{minipage}{.62\linewidth}
        %\begin{table*}
        \begin{tabular}{@{\hspace{0.1em}}c@{\hspace{0.2em}}|@{\hspace{0.2em}}c@{\hspace{0.7em}}c@{\hspace{0.7em}}c@{\hspace{0.3em}}c@{\hspace{0.1em}}|@{\hspace{0.2em}}c@{\hspace{0.7em}}c@{\hspace{0.7em}}c@{\hspace{0.3em}}c@{\hspace{0.1em}}}
            \hline
            \multirow{2}{*}{\textbf{Method}} & \multicolumn{4}{c|@{\hspace{0.2em}}}{\textbf{DynamicEarthNet}} & \multicolumn{4}{c}{\textbf{HRSCD}} \\
             & \textbf{BC} & \textbf{SC} & \textbf{SCS} & \textbf{mIoU} & \textbf{BC} & \textbf{SC} & \textbf{SCS} & \textbf{mIoU} \\ \hline
            \textbf{\textit{\underline{Bi-temporal SCD:}}} &  &  &  & \\
            Segformer      & 11.3 & 31.5 & 21.4 & 39.7 & \enskip 9.7 & 20.3 & 15.0 & 52.7 \\
            Swin + UperNet & 11.1 & 28.0 & 19.6 & 41.4 & & & \\
            SETR-PUP       & 10.7 & 21.9 & 16.3 & 35.2 & & & \\
            \textbf{\textit{\underline{Cond./Cross-modal SCD:}}} &  &  &  & \\
            Segformer      & 11.9 & 31.5 & 21.7 & 39.7 & \enskip 2.8 & 20.3 & 11.6 & 52.7 \\
            Swin + UperNet & 12.2 & 28.0 & 20.1 & 41.4 & & & \\
            SETR-PUP       & 10.8 & 21.9 & 16.4 & 35.2 & & & \\
            \hline
            \textbf{MapFormer}\,(cond.)       & 23.0 & 29.0 & 26.0 & 39.9 & 48.0 & 21.5 & 34.7 & 52.9 \\
            \textbf{MapFormer}\,(cross-mod.) & 20.4 & 30.7 & 25.5 & 40.3 & 45.6 & 21.7 & 33.5 & 49.9 \\
            \hline
        \end{tabular}
        \caption{Semantic change detection with semantic segmentation baselines and MapFormer. Segmentation baselines for bi-temporal and Conditional/Cross-modal SCD are identical models with the difference that $\hat{b}$ is computed via $\hat{m}^{(1)} == \hat{m}^{(2)}$ (bi-temporal) and via $m^{(1)} == \hat{m}^{(2)}$ (cond./cross-modal), respectively. Thus, only $BC$ and $SCS$ differ between the settings. Conditional and Cross-modal SCD are consolidated here as we assume the same set of training images both timesteps for a valid comparison.}
        \label{tab:semseg_baselines}
        %\end{table*}
    \end{minipage} 
    \hfill
    \begin{minipage}{0.37\linewidth}
        %\begin{table}
            %\centering
            \begin{tabular}{@{\hspace{0.2em}}c@{\hspace{0.2em}}|@{\hspace{0.3em}}c@{\hspace{0.6em}}c@{\hspace{0.3em}}|@{\hspace{0.6em}}c@{\hspace{0.6em}}c@{\hspace{0.3em}}}
            \hline
            \multirow{2}{*}{\textbf{Method}} & \multicolumn{2}{@{\hspace{0.2em}}c@{\hspace{0.6em}}|@{\hspace{0.6em}}}{\textbf{DynENet}} & \multicolumn{2}{@{\hspace{0.3em}}c@{\hspace{0.3em}}}{\textbf{HRSCD}} \\
              & \textbf{F1} & \textbf{IoU} & \textbf{F1} & \textbf{IoU} \\ \hline
            \textbf{\textit{\underline{Conditional BCD:}}} &  &  &  & \\ 
            %Classwise BCD         & & & & \\
            FHD+Concat          & 33.2 & 19.9 & 61.2 & 44.1\\
            ChangerEx+Concat    & 30.9 & 18.3 & 58.1 & 41.0 \\
            ChangeF.+Concat & 31.4 & 18.6 & 61.5 & 44.4 \\
            \textbf{MapFormer}$_{K=10}$                    & \textbf{38.0}   & \textbf{23.5}    & \textbf{64.5} & \textbf{47.7} \\
            \hline
            \end{tabular}
            \caption{Extensions of bi-temporal BCD methods to Conditional BCD. We concatenated encoded map features to the merge bi-temporal image features and trained with the exact same hyperparameters as in Table 2 in the paper.}
            \label{tab:cond_bcd_baselines}
        %\end{table}
    \end{minipage} 
\end{table*}
